System on Chip Rejuvenation in the Wake of Persistent Attacks

To cope with the ever increasing threats of dynamic and adaptive persistent attacks, Fault and Intrusion Tolerance (FIT) is being studied at the hardware level to increase critical systems resilience. Based on state-machine replication, FIT is known to be effective if replicas are compromised and fail independently. This requires different ways of diversification at the software and hardware levels. In this paper, we introduce the first hardware-based rejuvenation framework, we call Samsara, that allows for creating new computing cores (on which FIT replicas run) with diverse architectures. This is made possible by taking advantage of the programmable and reconfigurable features of MPSoC with an FPGA. A persistent attack that analyzes and exploits the vulnerability of a core will not be able to exploit it as rejuvenation to a different core architecture is made fast enough. We discuss the feasibility of this design, and we leave the empirical evaluations for future work.

==> biography.tex <==
% biography section
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-pics/ahmad}}]{Ahmad T Sheikh}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio-pics/paulo}}]{Paulo~Esteves-Verissimo}
Biography text here.
\end{IEEEbiography}

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
The proposed framework is being evaluated on Zynq Ultrascale+ class of evaluation boards from Xilinx (AMD). The  parameters of interest are: 1) how quickly the node(s) can be rejuvenated in the presence of persistent adversary, ideally, it should be small enough so as to outpace the persistent threat, 2) how the number of replicas can be dynamically changed based on the adaptive threat plane. Other important factors are the consensus time and the time taken by the newly created or rejuvenated CPU core to update its states.

==> related-work.tex <==
\section{Related Work}
\label{sec:related-work}

In this section we discuss how MPSoC systems are being deployed to accelerate the computational tasks in various classes of works. The avid reader is suggested to consult~\cite{Ines2020} for the motivation behind \emph{Midir} and how it proposes to solve the low-level malicious faults. 

In 2013 Xilinx introduced CPU+FPGA platform namely The Zynq SoC~\cite{Zynq7000SoC} that offers an ARM processing system and reconfigurable FPGA logic on the same chip. Later on, Zynq Ultrascale+ MPSoC and RFSoC were introduced with multiple ARM processing chips and improved FPGA architecture. Traditional FPGAs have been widely used for acceleration of computationally intensive tasks~\cite{ZynqMPSoC}. In 2019, Xilinx introduced Adaptive Compute Acceleration Platform called Versal. The Versal devices offer high-performance ARM cores, vector processors and an improved FPGA fabric. Twitch announced that they achieved speedup of up to 30-fold with the ability to deliver 120 frames per-second once they shifted from CPU implementation to FPGA~\cite{twitch2018}. Homomorphic computation implementation on FPGA showed 5 times improvement in the speed up as compared to the GPU implementation~\cite{Sinha2019HPCA}.

Microsoft announced the Project Catapult~\cite{Putnam2014ISCA} in which FPGAs and CPUs were incorporated in a node~\cite{Caulfield2016MICRO} and many nodes were connected with each other to form a network with the purpose to speed up the Bing web search engine. In 2015, Intel announced the acquisition of Altera~\cite{Intel2015} with the aim to integrate their Xeon CPUs and FPGAs on a single die. In 2016, Amazon Web Services (AWS) announced the adoption of Xilinx devices to accelerate the user's programs~\cite{Amazon2016}. Through \emph{AWS Shell} API, the users are able to interact the with an FPGA instance to upload their accelerator design.

Following the lines of Microsoft and Amazon, Baidu~\cite{Baidu2017}, Tencent~\cite{Tencent2018}, Huawei~\cite{Huawei2017} and Alibaba~\cite{Alibaba2017, Alibaba2017_2} soon followed the lead with FPGA acceleration in the cloud. In 2017, IBM introduced cloudFPGA~\cite{Abel2017HOTI} that consisted of 1024 FPGAs in a datacentre rack for large scale acceleration. This brief history highlights the adoption of domain-specific accelerators as a new direction of computer architecture by the industry.

FPGAs have also been extended to the cloud services. However, as opposed to CPU or GPU based services that provides isolation in the virtualized environment, FPGAs yet to have to address isolation primitives. Chen et. al.~\cite{Chen2014CCF} proposed a software stack that divides the FPGA resources into slots and user is granted access to these slots from their respective virtualized execution environment. \cite{Mikhail2017Access} proposed a runtime manager to provide an interface between the software threads and the FPGA based accelerators. The manager software runs on a soft processor core, receives requests from the user program and then program the accelerator with a partially-defined bitstream. Similarly, Suhaib et. al.~\cite{Suhaib2015} proposed a framework to manage the resources of reconfigurable accelerators in cloud. The software performs low-level communication through a diver and high-level through a hypervisor. The hypervisor selects the optimum region in the FGPA fabric for partial reconfiguration. Walder et. al.~\cite{Walder2004} proposed a similar approach to manage partial reconfiguration resources through a runtime environment. Based on Microsoft's Catapult~\cite{Putnam2014ISCA}, an FPGA operating system for cloud computing is proposed in~\cite{Zhang2017APSys} with the objective of managing accelerators and loading them to the partial reconfigurable region with the best matched template. 

Security and reliability has so far been ignored in the design and implementation of accelerators design. This may primarily be due to the unavailability of isolation and security primitives at the hardware level. Furkan~\cite{Furkan2020CSUR} provides as excellent survey on the trends of CPU+FPGA adoption, secure FPGA configuration, security of IP and secure shared use of FPGAs. As stated earlier, replication lies at the heart of an intrusion-tolerant system. Classical replication methods like selective replication and TMR~\cite{Sheikh2017TVLSI, Sheikh2017Integration}, DMR~\cite{Sheikh2018DMR} provides protection against manufacturing and accidental faults. Byzantine fault tolerant algorithms~\cite{BFT1982, PBFT1999} belong to the class of algorithms with the aim to tolerate both accidental and malicious faults. Faults are tolerated by reaching a consensus of $|Q|=2f+1$ out of $n=3f+1$ replicas. Architectural hybridization~\cite{Verissimo2006} proposes an additional trusted-trustworthy component with in the replicated realm to further reduce the size of $n$ and $Q$ to $2f+1$ and $f+1$, respectively. The trusted-trustworthy components provide tamper-proof computations of basic critical tasks. In this work we aim to build upon \emph{Midir}~\cite{Ines2020} to extend it in terms of variable number of replicas, faster rejuvenation of a selected replica and match the consensus process speed to the speed of NOC.

==> threat-model.tex <==
\section{Threat Model}
\label{sec:threat-model}
Threat model is similar to that of~\cite{Ines2020} where software faults are considered in hypervisor, firmware and in any software module. 
Hardware faults are considered with the following conditions: 1) they only occur with in a CPU core, 2) their effect is confined to the CPU core and will not cause the system wide chip failure. Tiles~\cite{Waingold1997} are the abstract placeholders of computational resources connected to each other through the Network-on-Chip (NOC) and memory controllers. Processing components like CPU, GPU and accelerators can be mapped into the tile abstraction. 

It is assumed that more than $f$ replicas can be compromised during the reference time $T_a$. In this case, number of CPU cores can be increased or decreased based on the adaptive threat plane. For persistent faults in time $T_a$, nodes can be rejuvenated fast enough so as to outpace the adversary. 
